The Compton-Pair telescope: A prototype for a next-generation MeV $\gamma$-ray observatory

The Compton Pair (ComPair) telescope is a prototype that aims to develop the necessary technologies for future medium energy gamma-ray missions and to design, build, and test the prototype in a gamma-ray beam and balloon flight. The ComPair team has built an instrument that consists of 4 detector subsystems: a double-sided silicon strip detector Tracker, a novel high-resolution virtual Frisch-grid cadmium zinc telluride Calorimeter, and a high-energy hodoscopic cesium iodide Calorimeter, all of which are surrounded by a plastic scintillator anti-coincidence detector. These subsystems together detect and characterize photons via Compton scattering and pair production, enable a veto of cosmic rays, and are a proof-of-concept for a space telescope with the same architecture. A future medium-energy gamma-ray mission enabled through ComPair will address many questions posed in the Astro2020 Decadal survey in both the New Messengers and New Physics and the Cosmic Ecosystems themes. In this contribution, we will give an overview of the ComPair project and steps forward to the balloon flight.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

